Phase-Shifted Pilot Design for NOMA-Empowered Uplink ISAC Systems

The deployment of multiple transmitters (TXs) in integrated sensing and communication (ISAC) networks necessitates efficient resource sharing to overcome the limitations of orthogonal allocation. While conventional interleaved (CI) pilots combined with non-orthogonal multiple access (NOMA) improve spectral efficiency (SE), they inherently compromise sensing resolution due to spectral sparsity, rendering the CI nulling (CIN) extension a strictly limited remedy. This paper proposes a phase-shifted (PS) pilot design and its novel PS nulling (PSN) variant to integrate a communication TX (CTX) over the PS-ISAC framework. The PSN variant strategically punctures sensing signals at CTX pilot locations to preserve initial channel estimates, enabling a dense data overlay. To resolve the resulting multi-TX interference, joint iterative interference cancellation (IIC) is adapted for non-nulling configurations and sequential IIC is adapted for nulling variants, optimizing for both detection robustness and convergence speed. Simulation results across varying STX densities and modulation orders demonstrate that the phase-shifted frameworks maintain sensing integrity while explicitly reducing receiver-side computational complexities by $18.8\%$ and $21.0\%$ against their respective interleaved baselines.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{UE}[UE]{user equipment}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{ISAC}[ISAC]{integrated sensing and communication}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{LS}[LS]{least-square}
\acrodef{MMSE}[MMSE]{minimum mean-square error}
\acrodef{BPSK}[BPSK]{binary phase shift keying}
\acrodef{CI-ISAC}[CI-ISAC]{conventional interleaved-ISAC}
\acrodef{CB-ISAC}[CB-ISAC]{conventional block-ISAC}
\acrodef{PS-ISAC}[PS-ISAC]{phase-shifted-ISAC}
\acrodef{APS-ISAC}[APS-ISAC]{adaptive PS-ISAC}
\acrodef{MSE}[MSE]{mean-square error}
\acrodef{NOMA}[NOMA]{non-orthogonal multiple access}
\acrodef{OOBE}[OOBE]{out-of-band emissions}
\acrodef{OFDMA}[OFDMA]{orthogonal frequency-division multiple access}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{FPR}[FPR]{full pilot ratio}
\acrodef{PR}[PR]{pilot ratio}
\acrodef{MA}[MA]{multiple access}
\acrodef{NGMA}[NGMA]{next-generation MA}
\acrodef{PRS}[PRS]{positioning RS}
\acrodef{UL}[UL]{uplink}
\acrodef{DL}[DL]{downlink}
\acrodef{CC}[CC]{computational complexity}
\acrodef{PC}[PC]{power constraints}
\acrodef{DMRS}[DMRS]{demodulation RS}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{SE}[SE]{spectral efficiency}
\acrodef{MED}[MED]{maximum excess delay}
\acrodef{LSE}[LSE]{least-square estimation}
\acrodef{TRX}[TRX]{transceiver}
\acrodef{TX}[TX]{transmitter}
\acrodef{RX}[RX]{receiver}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{XR}[XR]{extended reality}
\acrodef{IoT}[IoT]{Internet of things}
\acrodef{TF}[TF]{time-frequency}
\acrodef{CRB}[CRB]{Cramér–Rao bound}
\acrodef{MAC}[MAC]{multiple access channel}
\acrodef{CPI}[CPI]{coherent processing interval}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{PS}[PS]{phase-shifted}
\acrodef{SP}[S/P]{serial-to-parallel}
\acrodef{DAC}[DAC]{digital-to-analog conversion}
\acrodef{ADC}[ADC]{analog-to-digital conversion}
\acrodef{AIC}[AIC]{Akaike information criterion}
\acrodef{MDL}[MDL]{minimum description length}
\acrodef{RCS}[RCS]{radar cross section}
\acrodef{ICI}[ICI]{inter-carrier interference}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PDF}[PDF]{probability density function}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{CFAR}[CFAR]{constant false alarm rate}
\acrodef{LTE}[LTE]{long-term evolution}
\acrodef{5G}[5G]{fifth-generation}
\acrodef{6G}[6G]{sixth-generation}
\acrodef{NR}[NR]{new radio}
\acrodef{RF}[RF]{reciprocal filtering}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{UE}[UE]{user equipment}
\acrodef{BS}[BS]{base station}
\acrodef{IID}[IID]{independent and identically-distributed}
\acrodef{RS}[RS]{reference signal}
\acrodef{RSI}[RSI]{residual SI}
\acrodef{ZC}[ZC]{Zadoff-Chu}
\acrodef{CRLB}[CRLB]{Cramér-Rao lower bound}
\acrodef{RMSE}[RMSE]{root MSE}
\acrodef{SI}[SI]{self-interference}
\acrodef{INR}[INR]{interference-to-noise ratio}
\acrodef{circularly symmetric complex Gaussian}[CSCG]{CSCG}
\acrodef{APSP}[APSP]{adjustable phase-shifted pilots}
\acrodef{CDD}[CDD]{cyclic-delay diversity}
\acrodef{PN}[PN]{pseudo random}
\acrodef{NLoS}[NLoS]{non-line-of-sight}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{IIC}[IIC]{iterative interference cancellation}
\acrodef{NMSE}[NMSE]{normalized mean-square error}
\acrodef{PSN}[PSN]{PS nulling}
\acrodef{CIN}[CIN]{CI nulling}
\acrodef{BER}[BER]{bit error rate}
\acrodef{DFT}[DFT]{discrete Fourier transform}
\acrodef{STX}[STX]{sensing TX}
\acrodef{CTX}[CTX]{communication TX}
\acrodef{FMCW}[FMCW]{frequency modulated continuous wave}
\acrodef{CCI}[CCI]{co-channel interference}
\acrodef{OTFS}[OTFS]{orthogonal time frequency space}
\acrodef{CI}[CI]{conventional interleaved}
\acrodef{DD}[DD]{decision-directed}
\acrodef{TDM}[TDM]{time-division multiplexed}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
\acrodef{}[]{}
